Fractional viscoelastic models for power-law materials

Soft materials often exhibit a distinctive power-law viscoelastic response arising from broad distribution of time-scales present in their complex internal structure. A promising tool to accurately describe the rheological behaviour of soft materials is fractional calculus. However, its use in the scientific community remains limited due to the unusual notation and non-trivial properties of fractional operators. This review aims to provide a clear and accessible description of fractional viscoelastic models for a broad audience, and to demonstrate the ability of these models to deliver a unified approach for the characterisation of power-law materials. The use of a consistent framework for the analysis of rheological data would help classify the empirical behaviours of soft and biological materials, and better understand their response.

==> biblio.tex <==

@article{paszkowiak2003arterial,
  title={Arterial wall shear stress: observations from the bench to the bedside},
  author={Paszkowiak, Jacek J and Dardik, Alan},
  journal={Vascular and endovascular surgery},
  volume={37},
  number={1},
  pages={47--57},
  year={2003},
  publisher={Sage Publications Sage CA: Thousand Oaks, CA}
}

@article{lodish2000molecular,
  title={Molecular cell biology 4th edition},
  author={Lodish, Harvey and Berk, Arnold and Zipursky, S Lawrence and Matsudaira, Paul and Baltimore, David and Darnell, James},
  journal={National Center for Biotechnology Information{\~O}s Bookshelf},
  year={2000}
}

@article{heisenberg2013forces,
  title={Forces in tissue morphogenesis and patterning},
  author={Heisenberg, Carl-Philipp and Bella{\"\i}che, Yohanns},
  journal={Cell},
  volume={153},
  number={5},
  pages={948--962},
  year={2013},
  publisher={Elsevier}
}

@article{keller2003we,
  title={How we are shaped: the biomechanics of gastrulation},
  author={Keller, Ray and Davidson, Lance A and Shook, David R},
  journal={Differentiation},
  volume={71},
  number={3},
  pages={171--205},
  year={2003},
  publisher={Wiley Online Library}
}

@article{butler2009cell,
  title={Cell shape changes indicate a role for extrinsic tensile forces in Drosophila germ-band extension},
  author={Butler, Lucy C and Blanchard, Guy B and Kabla, Alexandre J and Lawrence, Nicola J and Welchman, David P and Mahadevan, L and Adams, Richard J and Sanson, Benedicte},
  journal={Nature cell biology},
  volume={11},
  number={7},
  pages={859},
  year={2009},
  publisher={Nature Publishing Group}
}

@article{cunningham2005role,
  title={The role of shear stress in the pathogenesis of atherosclerosis},
  author={Cunningham, Kristopher S and Gotlieb, Avrum I},
  journal={Laboratory investigation},
  volume={85},
  number={1},
  pages={9},
  year={2005},
  publisher={Nature Publishing Group}
}

@article{moulding2012excess,
  title={Excess F-actin mechanically impedes mitosis leading to cytokinesis failure in X-linked neutropenia by exceeding Aurora B kinase error correction capacity},
  author={Moulding, Dale A and Moeendarbary, Emad and Valon, Leo and Record, Julien and Charras, Guillaume T and Thrasher, Adrian J},
  journal={Blood},
  pages={blood--2012},
  year={2012},
  publisher={Am Soc Hematology}
}

@article{white2015lung,
  title={Lung extracellular matrix and fibroblast function},
  author={White, Eric S},
  journal={Annals of the American Thoracic Society},
  volume={12},
  number={Supplement 1},
  pages={S30--S33},
  year={2015},
  publisher={American Thoracic Society}
}

@article{jones2018nanoscale,
  title={Nanoscale dysregulation of collagen structure-function disrupts mechano-homeostasis and mediates pulmonary fibrosis},
  author={Jones, Mark G and Andriotis, Orestis G and Roberts, James JW and Lunn, Kerry and Tear, Victoria J and Cao, Lucy and Ask, Kjetil and Smart, David E and Bonfanti, Alessandra and Johnson, Peter and others},
  journal={eLife},
  volume={7},
  pages={e36354},
  year={2018},
  publisher={eLife Sciences Publications Limited}
}

@article{fritsch2010biomechanical,
  title={Are biomechanical changes necessary for tumour progression?},
  author={Fritsch, Anatol and H{\"o}ckel, Michael and Kiessling, Tobias and Nnetu, Kenechukwu David and Wetzel, Franziska and Zink, Mareike and K{\"a}s, Josef A},
  journal={Nature Physics},
  volume={6},
  number={10},
  pages={730},
  year={2010},
  publisher={Nature Publishing Group}
}

@article{guilak2014biomechanics,
  title={Biomechanics and mechanobiology in functional tissue engineering},
  author={Guilak, Farshid and Butler, David L and Goldstein, Steven A and Baaijens, Frank PT},
  journal={Journal of biomechanics},
  volume={47},
  number={9},
  pages={1933--1940},
  year={2014},
  publisher={Elsevier}
}

@article{nimeskern2013quantitative,
  title={Quantitative evaluation of mechanical properties in tissue-engineered auricular cartilage},
  author={Nimeskern, Luc and van Osch, Gerjo JVM and M{\"u}ller, Ralph and Stok, Kathryn S},
  journal={Tissue Engineering Part B: Reviews},
  volume={20},
  number={1},
  pages={17--27},
  year={2013},
  publisher={Mary Ann Liebert, Inc. 140 Huguenot Street, 3rd Floor New Rochelle, NY 10801 USA}
}

@article{chan2008scaffolding,
  title={Scaffolding in tissue engineering: general approaches and tissue-specific considerations},
  author={Chan, BP and Leong, KW},
  journal={European spine journal},
  volume={17},
  number={4},
  pages={467--479},
  year={2008},
  publisher={Springer}
}

@article{palacio2015quantitative,
  title={Quantitative diagnostics of soft tissue through viscoelastic characterization using time-based instrumented palpation},
  author={Palacio-Torralba, Javier and Hammer, Steven and Good, Daniel W and McNeill, S Alan and Stewart, Grant D and Reuben, Robert L and Chen, Yuhang},
  journal={journal of the mechanical behavior of biomedical materials},
  volume={41},
  pages={149--160},
  year={2015},
  publisher={Elsevier}
}

@article{phipps2005measurement,
  title={Measurement of tissue mechanical characteristics to distinguish between benign and malignant prostatic disease},
  author={Phipps, S and Yang, THJ and Habib, FK and Reuben, RL and McNeill, SA},
  journal={Urology},
  volume={66},
  number={2},
  pages={447--450},
  year={2005},
  publisher={Elsevier}
}

@article{remmerbach2009oral,
  title={Oral cancer diagnosis by mechanical phenotyping},
  author={Remmerbach, Torsten W and Wottawah, Falk and Dietrich, Julia and Lincoln, Bryan and Wittekind, Christian and Guck, Jochen},
  journal={Cancer research},
  volume={69},
  number={5},
  pages={1728--1732},
  year={2009},
  publisher={AACR}
}

@article{pant2011multiobjective,
  title={Multiobjective design optimisation of coronary stents},
  author={Pant, Sanjay and Limbert, Georges and Curzen, Nick P and Bressloff, Neil W},
  journal={Biomaterials},
  volume={32},
  number={31},
  pages={7755--7773},
  year={2011},
  publisher={Elsevier}
}

@article{bates2007linking,
  title={Linking parenchymal disease progression to changes in lung mechanical function by percolation},
  author={Bates, Jason HT and Davis, Gerald S and Majumdar, Arnab and Butnor, Kelly J and Suki, B{\'e}la},
  journal={American journal of respiratory and critical care medicine},
  volume={176},
  number={6},
  pages={617--623},
  year={2007},
  publisher={American Thoracic Society}
}

@article{odell1981mechanical,
  title={The mechanical basis of morphogenesis: I. Epithelial folding and invagination},
  author={Odell, Garrett M and Oster, George and Alberch, Pere and Burnside, Beth},
  journal={Developmental biology},
  volume={85},
  number={2},
  pages={446--462},
  year={1981},
  publisher={Elsevier}
}

@article{okuda2015vertex,
  title={Vertex dynamics simulations of viscosity-dependent deformation during tissue morphogenesis},
  author={Okuda, Satoru and Inoue, Yasuhiro and Eiraku, Mototsugu and Adachi, Taiji and Sasai, Yoshiki},
  journal={Biomechanics and modeling in mechanobiology},
  volume={14},
  number={2},
  pages={413--425},
  year={2015},
  publisher={Springer}
}

@article{rahimov2013cellular,
  title={Cellular and molecular mechanisms underlying muscular dystrophy},
  author={Rahimov, Fedik and Kunkel, Louis M},
  journal={J Cell Biol},
  volume={201},
  number={4},
  pages={499--510},
  year={2013},
  publisher={Rockefeller University Press}
}

@article{fabry2001scaling,
  title={Scaling the microrheology of living cells},
  author={Fabry, Ben and Maksym, Geoffrey N and Butler, James P and Glogauer, Michael and Navajas, Daniel and Fredberg, Jeffrey J},
  journal={Physical review letters},
  volume={87},
  number={14},
  pages={148102},
  year={2001},
  publisher={APS}
}

@article{desprat2005creep,
  title={Creep function of a single living cell},
  author={Desprat, Nicolas and Richert, Alain and Simeon, Jacqueline and Asnacios, Atef},
  journal={Biophysical journal},
  volume={88},
  number={3},
  pages={2224--2233},
  year={2005},
  publisher={Elsevier}
}

@article{bursac2005cytoskeletal,
  title={Cytoskeletal remodelling and slow dynamics in the living cell},
  author={Bursac, Predrag and Lenormand, Guillaume and Fabry, Ben and Oliver, Madavi and Weitz, David A and Viasnoff, Virgile and Butler, James P and Fredberg, Jeffrey J},
  journal={Nature materials},
  volume={4},
  number={7},
  pages={557},
  year={2005},
  publisher={Nature Publishing Group}
}

@article{guilak2000viscoelastic,
  title={Viscoelastic properties of the cell nucleus},
  author={Guilak, Farshid and Tedrow, John R and Burgkart, Rainer},
  journal={Biochemical and biophysical research communications},
  volume={269},
  number={3},
  pages={781--786},
  year={2000},
  publisher={Elsevier}
}

@article{caille2002contribution,
  title={Contribution of the nucleus to the mechanical properties of endothelial cells},
  author={Caille, Nathalie and Thoumine, Olivier and Tardy, Yanik and Meister, Jean-Jacques},
  journal={Journal of biomechanics},
  volume={35},
  number={2},
  pages={177--187},
  year={2002},
  publisher={Elsevier}
}

@article{hildebrandt1969comparison,
  title={Comparison of mathematical models for cat lung and viscoelastic balloon derived by Laplace transform methods from pressurevolume data},
  author={Hildebrandt, J},
  journal={The Bulletin of mathematical biophysics},
  volume={31},
  number={4},
  pages={651--667},
  year={1969},
  publisher={Springer}
}

@article{doubrovinski2017measurement,
  title={Measurement of cortical elasticity in Drosophila melanogaster embryos using ferrofluids},
  author={Doubrovinski, Konstantin and Swan, Michael and Polyakov, Oleg and Wieschaus, Eric F},
  journal={Proceedings of the National Academy of Sciences},
  volume={114},
  number={5},
  pages={1051--1056},
  year={2017},
  publisher={National Acad Sciences}
}

@article{fernandez2007shear,
  title={Shear rheology of a cell monolayer},
  author={Fern{\'a}ndez, Pablo and Heymann, Lutz and Ott, Albrecht and Aksel, Nuri and Pullarkat, Pramod A},
  journal={New Journal of Physics},
  volume={9},
  number={11},
  pages={419},
  year={2007},
  publisher={IOP Publishing}
}

@article{mizuno2007nonequilibrium,
  title={Nonequilibrium mechanics of active cytoskeletal networks},
  author={Mizuno, Daisuke and Tardin, Catherine and Schmidt, Christoph F and MacKintosh, Frederik C},
  journal={Science},
  volume={315},
  number={5810},
  pages={370--373},
  year={2007},
  publisher={American Association for the Advancement of Science}
}

@article{fletcher2010cell,
  title={Cell mechanics and the cytoskeleton},
  author={Fletcher, Daniel A and Mullins, R Dyche},
  journal={Nature},
  volume={463},
  number={7280},
  pages={485},
  year={2010},
  publisher={Nature Publishing Group}
}

@article{chancellor2010actomyosin,
  title={Actomyosin tension exerted on the nucleus through nesprin-1 connections influences endothelial cell adhesion, migration, and cyclic strain-induced reorientation},
  author={Chancellor, TJ and Lee, Jiyeon and Thodeti, Charles K and Lele, Tanmay},
  journal={Biophysical journal},
  volume={99},
  number={1},
  pages={115--123},
  year={2010},
  publisher={Elsevier}
}

@article{bardet2013pten,
  title={PTEN controls junction lengthening and stability during cell rearrangement in epithelial tissue},
  author={Bardet, Pierre-Luc and Guirao, Boris and Paoletti, Camille and Serman, Fanny and L{\'e}opold, Valentine and Bosveld, Floris and Goya, Y{\^u}ki and Mirouse, Vincent and Graner, Fran{\c{c}}ois and Bella{\"\i}che, Yohanns},
  journal={Developmental cell},
  volume={25},
  number={5},
  pages={534--546},
  year={2013},
  publisher={Elsevier}
}

@article{harris2014formation,
  title={Formation of adherens junctions leads to the emergence of a tissue-level tension in epithelial monolayers},
  author={Harris, Andrew R and Daeden, Alicia and Charras, Guillaume T},
  journal={J Cell Sci},
  pages={jcs--142349},
  year={2014},
  publisher={The Company of Biologists Ltd}
}

@article{guevorkian2010aspiration,
  title={Aspiration of biological viscoelastic drops},
  author={Guevorkian, Karine and Colbert, Marie-Jos{\'e}e and Durth, M{\'e}lanie and Dufour, Sylvie and Brochard-Wyart, Fran{\c{c}}oise},
  journal={Physical review letters},
  volume={104},
  number={21},
  pages={218101},
  year={2010},
  publisher={APS}
}

@article{clement2017viscoelastic,
  title={Viscoelastic dissipation stabilizes cell shape changes during tissue morphogenesis},
  author={Cl{\'e}ment, Rapha{\"e}l and Dehapiot, Beno{\^\i}t and Collinet, Claudio and Lecuit, Thomas and Lenne, Pierre-Fran{\c{c}}ois},
  journal={Current Biology},
  volume={27},
  number={20},
  pages={3132--3142},
  year={2017},
  publisher={Elsevier}
}

@article{alcaraz2003microrheology,
  title={Microrheology of human lung epithelial cells measured by atomic force microscopy},
  author={Alcaraz, Jordi and Buscemi, Lara and Grabulosa, Mireia and Trepat, Xavier and Fabry, Ben and Farr{\'e}, Ramon and Navajas, Daniel},
  journal={Biophysical journal},
  volume={84},
  number={3},
  pages={2071--2079},
  year={2003},
  publisher={Elsevier}
}

@article{plodinec2012nanomechanical,
  title={The nanomechanical signature of breast cancer},
  author={Plodinec, Marija and Loparic, Marko and Monnier, Christophe A and Obermann, Ellen C and Zanetti-Dallenbach, Rosanna and Oertle, Philipp and Hyotyla, Janne T and Aebi, Ueli and Bentires-Alj, Mohamed and Lim, Roderick YH and others},
  journal={Nature nanotechnology},
  volume={7},
  number={11},
  pages={757},
  year={2012},
  publisher={Nature Publishing Group}
}

@article{moreno2010stress,
  title={Stress relaxation and creep on living cells with the atomic force microscope: a means to calculate elastic moduli and viscosities of cell components},
  author={Moreno-Flores, Susana and Benitez, Rafael and dM Vivanco, Mar{\'\i}a and Toca-Herrera, Jos{\'e} Luis},
  journal={Nanotechnology},
  volume={21},
  number={44},
  pages={445101},
  year={2010},
  publisher={IOP Publishing}
}

@article{darling2006viscoelastic,
  title={Viscoelastic properties of zonal articular chondrocytes measured by atomic force microscopy},
  author={Darling, EM and Zauscher, S and Guilak, F},
  journal={Osteoarthritis and cartilage},
  volume={14},
  number={6},
  pages={571--579},
  year={2006},
  publisher={Elsevier}
}

@article{bausch1999measurement,
  title={Measurement of local viscoelasticity and forces in living cells by magnetic tweezers},
  author={Bausch, Andreas R and M{\"o}ller, Winfried and Sackmann, Erich},
  journal={Biophysical journal},
  volume={76},
  number={1},
  pages={573--579},
  year={1999},
  publisher={Elsevier}
}

@article{roylance2001engineering,
  title={Engineering viscoelasticity},
  author={Roylance, David},
  journal={Department of Materials Science and Engineering--Massachusetts Institute of Technology, Cambridge MA},
  volume={2139},
  pages={1--37},
  year={2001}
}

@book{bland2016theory,
  title={The theory of linear viscoelasticity},
  author={Bland, David Russell},
  year={2016},
  publisher={Courier Dover Publications}
}

@book{findley2013creep,
  title={Creep and relaxation of nonlinear viscoelastic materials},
  author={Findley, William N and Davis, Francis A},
  year={2013},
  publisher={Courier Corporation}
}

@article{harris2012characterizing,
  title={Characterizing the mechanics of cultured cell monolayers},
  author={Harris, Andrew R and Peter, Loic and Bellis, Julien and Baum, Buzz and Kabla, Alexandre J and Charras, Guillaume T},
  journal={Proceedings of the National Academy of Sciences},
  volume={109},
  number={41},
  pages={16449--16454},
  year={2012},
  publisher={National Acad Sciences}
}

@article{halldin2014constitutive,
  title={On a constitutive material model to capture time dependent behavior of cortical bone},
  author={Halldin, Anders and Ander, Mats and Jacobsson, Magnus and Hansson, Stig},
  journal={World Journal of Mechanics},
  volume={4},
  number={11},
  pages={348},
  year={2014},
  publisher={Scientific Research Publishing}
}

@article{bembey2006viscoelastic,
  title={Viscoelastic properties of bone as a function of hydration state determined by nanoindentation},
  author={Bembey, AK and Oyen, ML and Bushby, AJ and Boyde, A},
  journal={Philosophical Magazine},
  volume={86},
  number={33-35},
  pages={5691--5703},
  year={2006},
  publisher={Taylor \& Francis}
}

@article{efremov2017measuring,
  title={Measuring nanoscale viscoelastic parameters of cells directly from AFM force-displacement curves},
  author={Efremov, Yuri M and Wang, Wen-Horng and Hardy, Shana D and Geahlen, Robert L and Raman, Arvind},
  journal={Scientific reports},
  volume={7},
  number={1},
  pages={1541},
  year={2017},
  publisher={Nature Publishing Group}
}

@inproceedings{wang2016modeling,
  title={Modeling and analysis of mechanical properties of single cells},
  author={Wang, Bo and Wang, Wenxue and Wang, Yuechao and Liu, Lianqing},
  booktitle={Nano/Molecular Medicine and Engineering (NANOMED), 2016 IEEE 10th International Conference on},
  pages={51--54},
  year={2016},
  organization={IEEE}
}

@article{rianna2017comparison,
  title={Comparison of viscoelastic properties of cancer and normal thyroid cells on different stiffness substrates},
  author={Rianna, Carmela and Radmacher, Manfred},
  journal={European Biophysics Journal},
  volume={46},
  number={4},
  pages={309--324},
  year={2017},
  publisher={Springer}
}

@article{kobayashi2017simple,
  title={Simple empirical model for identifying rheological properties of soft biological tissues},
  author={Kobayashi, Yo and Tsukune, Mariko and Miyashita, Tomoyuki and Fujie, Masakatsu G},
  journal={Physical Review E},
  volume={95},
  number={2},
  pages={022418},
  year={2017},
  publisher={APS}
}

@article{huber2015cytoskeletal,
  title={Cytoskeletal crosstalk: when three different personalities team up},
  author={Huber, Florian and Boire, Adeline and Lopez, Magdalena Preciado and Koenderink, Gijsje H},
  journal={Current opinion in cell biology},
  volume={32},
  pages={39--47},
  year={2015},
  publisher={Elsevier}
}

@article{bonakdar2016mechanical,
  title={Mechanical plasticity of cells},
  author={Bonakdar, Navid and Gerum, Richard and Kuhn, Michael and Sp{\"o}rrer, Marina and Lippert, Anna and Schneider, Werner and Aifantis, Katerina E and Fabry, Ben},
  journal={Nature materials},
  volume={15},
  number={10},
  pages={1090},
  year={2016},
  publisher={Nature Publishing Group}
}


@article{khalilgharibi,
  title={Stress relaxation in epithelial monolayers is controlled by the actomyosin cortex},
  author={Khalilgharibi, Nargess and Fouchard, Jonathan and Asadipour, Nina and Barrientos, Ricardo and Duda, Maria and Bonfanti, Alessandra and Yonis, Amina and Harris, Andrew and Mosaffa, Payman and Fujita, Yasuyuki and others},
  journal={Nature Physics},
  pages={1},
  year={2019},
  publisher={Nature Publishing Group}
}



@article{winter1986analysis,
  title={Analysis of linear viscoelasticity of a crosslinking polymer at the gel point},
  author={Winter, H Henning and Chambon, Francois},
  journal={Journal of rheology},
  volume={30},
  number={2},
  pages={367--382},
  year={1986},
  publisher={SOR}
}

@article{craiem2008fractional,
  title={Fractional-order viscoelasticity applied to describe uniaxial stress relaxation of human arteries},
  author={Craiem, Damian and Rojo, Francisco J and Atienza, Jose Miguel and Armentano, Ricardo L and Guinea, Gustavo V},
  journal={Physics in Medicine \& Biology},
  volume={53},
  number={17},
  pages={4543},
  year={2008},
  publisher={IOP Publishing}
}

@article{heymans2008dynamic,
  title={Dynamic measurements in long-memory materials: fractional calculus evaluation of approach to steady state},
  author={Heymans, Nicole},
  journal={Journal of Vibration and Control},
  volume={14},
  number={9-10},
  pages={1587--1596},
  year={2008},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{craiem2010fractional,
  title={Fractional order models of viscoelasticity as an alternative in the analysis of red blood cell (RBC) membrane mechanics},
  author={Craiem, Damian and Magin, Richard L},
  journal={Physical biology},
  volume={7},
  number={1},
  pages={013001},
  year={2010},
  publisher={IOP Publishing}
}

@article{nicolas2018biomechanical,
  title={Biomechanical characterization of ex vivo human brain using ultrasound shear wave spectroscopy},
  author={Nicolas, Emmanuel and Calle, Samuel and Nicolle, St{\'e}phane and Mitton, David and Remenieras, Jean-Pierre},
  journal={Ultrasonics},
  volume={84},
  pages={119--125},
  year={2018},
  publisher={Elsevier}
}

@article{bouzid2018computing,
  title={Computing the linear viscoelastic properties of soft gels using an Optimally Windowed Chirp protocol},
  author={Bouzid, Mehdi and Keshavarz, Bavand and Geri, Michela and Divoux, Thibaut and Del Gado, Emanuela and McKinley, Gareth H},
  journal={arXiv preprint arXiv:1805.07987},
  year={2018}
}

@article{carmichael2015fractional,
  title={The fractional viscoelastic response of human breast tissue cells},
  author={Carmichael, B and Babahosseini, H and Mahmoodi, SN and Agah, M},
  journal={Physical biology},
  volume={12},
  number={4},
  pages={046001},
  year={2015},
  publisher={IOP Publishing}
}

@article{alcoutlabi1998application,
  title={Application of fractional calculus to viscoelastic behaviour modelling and to the physical ageing phenomenon in glassy amorphous polymers},
  author={Alcoutlabi, M and Martinez-Vega, J},
  journal={Polymer},
  volume={39},
  number={25},
  pages={6269--6277},
  year={1998},
  publisher={Elsevier}
}

@article{kohandel2005frequency,
  title={Frequency dependence of complex moduli of brain tissue using a fractional Zener model},
  author={Kohandel, M and Sivaloganathan, S and Tenti, G and Darvish, K},
  journal={Physics in Medicine \& Biology},
  volume={50},
  number={12},
  pages={2799},
  year={2005},
  publisher={IOP Publishing}
}

@article{yu2016fractional,
  title={Fractional modeling of viscoelasticity in 3D cerebral arteries and aneurysms},
  author={Yu, Yue and Perdikaris, Paris and Karniadakis, George Em},
  journal={Journal of computational physics},
  volume={323},
  pages={219--242},
  year={2016},
  publisher={Elsevier}
}

@article{fraldi2015frequency,
  title={A frequency-based hypothesis for mechanically targeting and selectively attacking cancer cells},
  author={Fraldi, M and Cugno, A and Deseri, Luca and Dayal, K and Pugno, NM},
  journal={Journal of The Royal Society Interface},
  volume={12},
  number={111},
  pages={20150656},
  year={2015},
  publisher={The Royal Society}
}

@article{hemmer2009role,
  title={Role of cytoskeletal components in stress-relaxation behavior of adherent vascular smooth muscle cells},
  author={Hemmer, Jason D and Nagatomi, Jiro and Wood, Scott T and Vertegel, Alexey A and Dean, Delphine and LaBerge, Martine},
  journal={Journal of biomechanical engineering},
  volume={131},
  number={4},
  pages={041001},
  year={2009},
  publisher={American Society of Mechanical Engineers}
}

@article{hoffman2006consensus,
  title={The consensus mechanics of cultured mammalian cells},
  author={Hoffman, Brenton D and Massiera, Gladys and Van Citters, Kathleen M and Crocker, John C},
  journal={Proceedings of the National Academy of Sciences},
  volume={103},
  number={27},
  pages={10259--10264},
  year={2006},
  publisher={National Acad Sciences}
}

@article{bagley1983theoretical,
  title={A theoretical basis for the application of fractional calculus to viscoelasticity},
  author={Bagley, Ronald L and Torvik, PJ},
  journal={Journal of Rheology},
  volume={27},
  number={3},
  pages={201--210},
  year={1983},
  publisher={SOR}
}

@article{bagley1989power,
  title={Power law and fractional calculus model of viscoelasticity},
  author={Bagley, Ronald L},
  journal={AIAA journal},
  volume={27},
  number={10},
  pages={1412--1417},
  year={1989}
}

@article{kiss2004viscoelastic,
  title={Viscoelastic characterization of in vitro canine tissue},
  author={Kiss, Miklos Z and Varghese, Tomy and Hall, Timothy J},
  journal={Physics in Medicine \& Biology},
  volume={49},
  number={18},
  pages={4207},
  year={2004},
  publisher={IOP Publishing}
}

@article{suki1994lung,
  title={Lung tissue viscoelasticity: a mathematical framework and its molecular basis},
  author={Suki, Bela and Barabasi, ALBERT-LASZL and Lutchen, KENNETH R},
  journal={Journal of Applied Physiology},
  volume={76},
  number={6},
  pages={2749--2759},
  year={1994}
}

@article{mino2016linear,
  title={Linear and nonlinear fractional hereditary constitutive laws of asphalt mixtures},
  author={Mino, Gaetano Di and Airey, Gordon and Di Paola, Mario and Pinnola, Francesco Paolo and D’Angelo, Giacomo and Presti, Davide Lo},
  journal={Journal of Civil Engineering and Management},
  volume={22},
  number={7},
  pages={882--889},
  year={2016},
  publisher={Taylor \& Francis}
}


@article{gayer2009effects,
  title={The effects of mechanical forces on intestinal physiology and pathology},
  author={Gayer, Christopher P and Basson, Marc D},
  journal={Cellular signalling},
  volume={21},
  number={8},
  pages={1237--1244},
  year={2009},
  publisher={Elsevier}
}

@article{blair1942subjective,
  title={The subjective conception of the firmness of soft materials},
  author={Blair, GW Scott and Coppen, FMV},
  journal={The American Journal of Psychology},
  pages={215--229},
  year={1942},
  publisher={JSTOR}
}

@article{blair1947role,
  title={The role of psychophysics in rheology},
  author={Blair, GW Scott},
  journal={Journal of Colloid Science},
  volume={2},
  number={1},
  pages={21--32},
  year={1947},
  publisher={Elsevier}
}

@article{di2011visco,
  title={Visco-elastic behavior through fractional calculus: an easier method for best fitting experimental results},
  author={Di Paola, Mi and Pirrotta, A and Valenza, A},
  journal={Mechanics of materials},
  volume={43},
  number={12},
  pages={799--806},
  year={2011},
  publisher={Elsevier}
}

@article{mainardi2008,
  title={Fractional Calculus: Integral and Differential Equations of Fractional Order},
  author={Gorenflo, R and Mainardi, F},
  journal={Fractals and Fractional Calculus in Continuum Mechanics},
  volume={1},
  number={1},
  pages={223-276},
  year={2008},
  publisher={Springer}
}

@article{mainardi2014propMittLeff,
  title = {On Some Properties of the {Mittag}-{Leffler} Function {$E_\alpha$($-t^\alpha$)}, Completely Monotone for T>0 with 0<$\alpha$<1},
  doi = {10.3934/dcdsb.2014.19.2267},
  journal = {Discrete \& Continuous Dynamical Systems - B2014, Volume 19, Pages 2267-2278},
  url = {http://www.aimsciences.org/journals/displayArticlesnew.jsp?paperID=10192},
  author = {Mainardi, Francesco},
  year = {2014},
}

@article{deseri2013power,
  title={Power-law hereditariness of hierarchical fractal bones},
  author={Deseri, Luca and Paola, Mario Di and Zingales, Massimiliano and Pollaci, Pietro},
  journal={International journal for numerical methods in biomedical engineering},
  volume={29},
  number={12},
  pages={1338--1360},
  year={2013},
  publisher={Wiley Online Library}
}

@inproceedings{jaishankar2013power,
  title={Power-law rheology in the bulk and at the interface: quasi-properties and fractional constitutive equations},
  author={Jaishankar, Aditya and McKinley, Gareth H},
  booktitle={Proc. R. Soc. A},
  volume={469},
  pages={20120284},
  year={2013},
  organization={The Royal Society}
}

@article{waters2012mechanobiology,
  title={Mechanobiology in lung epithelial cells: measurements, perturbations, and responses},
  author={Waters, Christopher M and Roan, Esra and Navajas, Daniel},
  journal={Comprehensive Physiology},
  year={2012},
  publisher={Wiley Online Library}
}


@article{moeendarbary2013cytoplasm,
  title={The cytoplasm of living cells behaves as a poroelastic material},
  author={Moeendarbary, Emad and Valon, L{\'e}o and Fritzsche, Marco and Harris, Andrew R and Moulding, Dale A and Thrasher, Adrian J and Stride, Eleanor and Mahadevan, L and Charras, Guillaume T},
  journal={Nature materials},
  volume={12},
  number={3},
  pages={253},
  year={2013},
  publisher={Europe PMC Funders}
}

@article{harris2013generating,
  title={Generating suspended cell monolayers for mechanobiological studies},
  author={Harris, Andrew R and Bellis, Julien and Khalilgharibi, Nargess and Wyatt, Tom and Baum, Buzz and Kabla, Alexandre J and Charras, Guillaume T},
  journal={Nature protocols},
  volume={8},
  number={12},
  pages={2516},
  year={2013},
  publisher={Nature Publishing Group}
}

@article{wyatt2016question,
  title={A question of time: tissue adaptation to mechanical forces},
  author={Wyatt, Tom and Baum, Buzz and Charras, Guillaume},
  journal={Current opinion in cell biology},
  volume={38},
  pages={68--73},
  year={2016},
  publisher={Elsevier}
}

@article{stewart2012tracking,
  title={Tracking mechanics and volume of globular cells with atomic force microscopy using a constant-height clamp},
  author={Stewart, Martin P and Toyoda, Yusuke and Hyman, Anthony A and M{\"u}ller, Daniel J},
  journal={nature protocols},
  volume={7},
  number={1},
  pages={143},
  year={2012},
  publisher={Nature Publishing Group}
}

@article{solomonow2003muscular,
  title={Muscular dysfunction elicited by creep of lumbar viscoelastic tissue},
  author={Solomonow, M and Baratta, RV and Zhou, B-H and Burger, E and Zieske, A and Gedalia, A},
  journal={Journal of Electromyography and Kinesiology},
  volume={13},
  number={4},
  pages={381--396},
  year={2003},
  publisher={Elsevier}
}

@article{hoffman2009cell,
  title={Cell mechanics: dissecting the physical responses of cells to force},
  author={Hoffman, Brenton D and Crocker, John C},
  journal={Annual review of biomedical engineering},
  volume={11},
  pages={259--288},
  year={2009},
  publisher={Annual Reviews}
}

@article{trepat2008universality,
  title={Universality in cell mechanics},
  author={Trepat, Xavier and Lenormand, Guillaume and Fredberg, Jeffrey J},
  journal={Soft Matter},
  volume={4},
  number={9},
  pages={1750--1759},
  year={2008},
  publisher={Royal Society of Chemistry}
}

@article{fischer2016rheology,
  title={Rheology of the active cell cortex in mitosis},
  author={Fischer-Friedrich, Elisabeth and Toyoda, Yusuke and Cattin, Cedric J and M{\"u}ller, Daniel J and Hyman, Anthony A and J{\"u}licher, Frank},
  journal={Biophysical journal},
  volume={111},
  number={3},
  pages={589--600},
  year={2016},
  publisher={Elsevier}
}

@article{desprat2006microplates,
  title={Microplates-based rheometer for a single living cell},
  author={Desprat, N and Guiroy, A and Asnacios, A},
  journal={Review of scientific instruments},
  volume={77},
  number={5},
  pages={055111},
  year={2006},
  publisher={AIP}
}

@article{blair1949vi,
  title={VI. An application of the theory of quasi-properties to the treatment of anomalous strain-stress relations},
  author={Blair, GW Scott and Caffyn, JE},
  journal={The London, Edinburgh, and Dublin Philosophical Magazine and Journal of Science},
  volume={40},
  number={300},
  pages={80--94},
  year={1949},
  publisher={Taylor \& Francis}
}


@article{zhou2010power,
  title={Power-law rheology analysis of cells undergoing micropipette aspiration},
  author={Zhou, EH and Quek, ST and Lim, CT},
  journal={Biomechanics and modeling in mechanobiology},
  volume={9},
  number={5},
  pages={563--572},
  year={2010},
  publisher={Springer}
}

@article{zhou2011creep,
  title={A creep constitutive model for salt rock based on fractional derivatives},
  author={Zhou, HW and Wang, CP and Han, BB and Duan, ZQ},
  journal={International Journal of Rock Mechanics and Mining Sciences},
  volume={48},
  number={1},
  pages={116--121},
  year={2011},
  publisher={Elsevier}
}


@article{bouras2018non,
  title={A non-linear thermo-viscoelastic rheological model based on fractional derivatives for high temperature creep in concrete},
  author={Bouras, Yanni and Zorica, Du{\v{s}}an and Atanackovi{\'c}, Teodor M and Vrcelj, Zora},
  journal={Applied Mathematical Modelling},
  volume={55},
  pages={551--568},
  year={2018},
  publisher={Elsevier}
}

@article{barpi2002creep,
  title={Creep and fracture in concrete: a fractional order rate approach},
  author={Barpi, Fabrizio and Valente, Silvio},
  journal={Engineering Fracture Mechanics},
  volume={70},
  number={5},
  pages={611--623},
  year={2002},
  publisher={Elsevier}
}

@article{fredberg1989imperfect,
  title={On the imperfect elasticity of lung tissue},
  author={Fredberg, Jeffrey J and Stamenovic, Dimitrije},
  journal={Journal of applied physiology},
  volume={67},
  number={6},
  pages={2408--2419},
  year={1989}
}

@article{rother2015cytoskeleton,
  title={Cytoskeleton remodelling of confluent epithelial cells cultured on porous substrates},
  author={Rother, Jan and B{\"u}chsensch{\"u}tz-G{\"o}beler, Matthias and N{\"o}ding, Helen and Steltenkamp, Siegfried and Samwer, Konrad and Janshoff, Andreas},
  journal={Journal of The Royal Society Interface},
  volume={12},
  number={103},
  pages={20141057},
  year={2015},
  publisher={The Royal Society}
}

@article{cai2013quantifying,
  title={Quantifying cell-to-cell variation in power-law rheology},
  author={Cai, PingGen and Mizutani, Yusuke and Tsuchiya, Masahiro and Maloney, John M and Fabry, Ben and Van Vliet, Krystyn J and Okajima, Takaharu},
  journal={Biophysical journal},
  volume={105},
  number={5},
  pages={1093--1102},
  year={2013},
  publisher={Elsevier}
}

@article{fabry2003time,
  title={Time scale and other invariants of integrative mechanical behavior in living cells},
  author={Fabry, Ben and Maksym, Geoffrey N and Butler, James P and Glogauer, Michael and Navajas, Daniel and Taback, Nathan A and Millet, Emil J and Fredberg, Jeffrey J},
  journal={Physical Review E},
  volume={68},
  number={4},
  pages={041914},
  year={2003},
  publisher={APS}
}

@article{smith2005probing,
  title={Probing the viscoelastic behavior of cultured airway smooth muscle cells with atomic force microscopy: stiffening induced by contractile agonist},
  author={Smith, Benjamin A and Tolloczko, Barbara and Martin, James G and Gr{\"u}tter, Peter},
  journal={Biophysical journal},
  volume={88},
  number={4},
  pages={2994--3007},
  year={2005},
  publisher={Elsevier}
}


@article{pullarkat2007rheological,
  title={Rheological properties of the eukaryotic cell cytoskeleton},
  author={Pullarkat, Pramod A and Fern{\'a}ndez, Pablo A and Ott, Albrecht},
  journal={Physics Reports},
  volume={449},
  number={1-3},
  pages={29--53},
  year={2007},
  publisher={Elsevier}
}

@article{deng2006fast,
  title={Fast and slow dynamics of the cytoskeleton},
  author={Deng, Linhong and Trepat, Xavier and Butler, James P and Millet, Emil and Morgan, Kathleen G and Weitz, David A and Fredberg, Jeffrey J},
  journal={Nature materials},
  volume={5},
  number={8},
  pages={636},
  year={2006},
  publisher={Nature Publishing Group}
}

@article{schiessel1995generalized,
  title={Generalized viscoelastic models: their fractional equations with solutions},
  author={Schiessel, H and Metzler, R and Blumen, A and Nonnenmacher, TF},
  journal={Journal of physics A: Mathematical and General},
  volume={28},
  number={23},
  pages={6567},
  year={1995},
  publisher={IOP Publishing}
}


@article{subramanian2006linear,
  title={Linear viscoelastic properties of regular-and reduced-fat pasteurized process cheese during heating and cooling},
  author={Subramanian, R and Muthukumarappan, K and Gunasekaran, S},
  journal={International Journal of Food Properties},
  volume={9},
  number={3},
  pages={377--393},
  year={2006},
  publisher={Taylor \& Francis}
}

@article{siviello2015analysis,
  title={Analysis of linear viscoelastic behaviour of alginate gels: effects of inner relaxation, water diffusion, and syneresis},
  author={Siviello, Ciro and Greco, Francesco and Larobina, Domenico},
  journal={Soft matter},
  volume={11},
  number={30},
  pages={6045--6054},
  year={2015},
  publisher={Royal Society of Chemistry}
}

@article{zhang2008quantitative,
  title={Quantitative characterization of viscoelastic properties of human prostate correlated with histology},
  author={Zhang, Man and Nigwekar, Priya and Castaneda, Benjamin and Hoyt, Kenneth and Joseph, Jean V and di Sant'Agnese, Anthony and Messing, Edward M and Strang, John G and Rubens, Deborah J and Parker, Kevin J},
  journal={Ultrasound in medicine \& biology},
  volume={34},
  number={7},
  pages={1033--1042},
  year={2008},
  publisher={Elsevier}
}

@article{li2016viscoelastic,
  title={Viscoelastic-plastic behavior of single tomato mesocarp cells in high speed compression-holding tests},
  author={Li, Zhiguo and Zhang, Zhibing and Thomas, Colin},
  journal={Innovative Food Science \& Emerging Technologies},
  volume={34},
  pages={44--50},
  year={2016},
  publisher={Elsevier}
}

@article{shahin2018mechanical,
  title={Mechanical, material, and biological study of a PCL/bioactive glass bone scaffold: Importance of viscoelasticity},
  author={Shahin-Shamsabadi, Alireza and Hashemi, Ata and Tahriri, Mohammadreza and Bastami, Farshid and Salehi, Majid and Abbas, Fatemeh Mashhadi},
  journal={Materials Science and Engineering: C},
  volume={90},
  pages={280--288},
  year={2018},
  publisher={Elsevier}
}

@article{shen2011viscoelastic,
  title={Viscoelastic properties of isolated collagen fibrils},
  author={Shen, Zhilei Liu and Kahn, Harold and Ballarini, Roberto and Eppell, Steven J},
  journal={Biophysical journal},
  volume={100},
  number={12},
  pages={3008--3015},
  year={2011},
  publisher={Elsevier}
}

@article{dai2015model,
  title={A model of lung parenchyma stress relaxation using fractional viscoelasticity},
  author={Dai, Zoujun and Peng, Ying and Mansy, Hansen A and Sandler, Richard H and Royston, Thomas J},
  journal={Medical engineering \& physics},
  volume={37},
  number={8},
  pages={752--758},
  year={2015},
  publisher={Elsevier}
}

@article{perdikaris2014fractional,
  title={Fractional-order viscoelasticity in one-dimensional blood flow models},
  author={Perdikaris, Paris and Karniadakis, George Em},
  journal={Annals of biomedical engineering},
  volume={42},
  number={5},
  pages={1012--1023},
  year={2014},
  publisher={Springer}
}

@article{cai2017temporal,
  title={Temporal variation in single-cell power-law rheology spans the ensemble variation of cell population},
  author={Cai, PingGen and Takahashi, Ryosuke and Kuribayashi-Shigetomi, Kaori and Subagyo, Agus and Sueoka, Kazuhisa and Maloney, John M and Van Vliet, Krystyn J and Okajima, Takaharu},
  journal={Biophysical journal},
  volume={113},
  number={3},
  pages={671--678},
  year={2017},
  publisher={Elsevier}
}

@article{serwane2017vivo,
  title={In vivo quantification of spatially varying mechanical properties in developing tissues},
  author={Serwane, Friedhelm and Mongera, Alessandro and Rowghanian, Payam and Kealhofer, David A and Lucio, Adam A and Hockenbery, Zachary M and Camp{\`a}s, Otger},
  journal={Nature methods},
  volume={14},
  number={2},
  pages={181},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{pollack2001cell,
  title={Is the cell a gel—and why does it matter?},
  author={Pollack, Gerald H},
  journal={The Japanese journal of physiology},
  volume={51},
  number={6},
  pages={649--660},
  year={2001},
  publisher={Physiological Society of Japan}
}

@article{aime2018power,
  title={Power law viscoelasticity of a fractal colloidal gel},
  author={Aime, Stefano and Cipelletti, Luca and Ramos, Laurence},
  journal={Journal of Rheology},
  volume={62},
  number={6},
  pages={1429--1441},
  year={2018},
  publisher={The Society of Rheology}
}

@article{zhang2018modeling,
  title={Modeling ramp-hold indentation measurements based on Kelvin--Voigt fractional derivative model},
  author={Zhang, Hongmei and zhe Zhang, Qing and Ruan, Litao and Duan, Junbo and Wan, Mingxi and Insana, Michael F},
  journal={Measurement Science and Technology},
  volume={29},
  number={3},
  pages={035701},
  year={2018},
  publisher={IOP Publishing}
}

@article{choudhury2012forced,
  title={Forced spreading and rheology of starch gel: Viscoelastic modeling with fractional calculus},
  author={Choudhury, Moutushi Dutta and Chandra, Subrata and Nag, Soma and Das, Shantanu and Tarafdar, Sujata},
  journal={Colloids and Surfaces A: Physicochemical and Engineering Aspects},
  volume={407},
  pages={64--70},
  year={2012},
  publisher={Elsevier}
}

@article{chen2004dynamic,
  title={Dynamic mechanical properties of agarose gels modeled by a fractional derivative model},
  author={Chen, Qingshan and Suki, Bela and An, Kai-Nan},
  journal={Journal of biomechanical engineering},
  volume={126},
  number={5},
  pages={666--671},
  year={2004},
  publisher={American Society of Mechanical Engineers}
}

@article{meral2010fractional,
  title={Fractional calculus in viscoelasticity: an experimental study},
  author={Meral, FC and Royston, TJ and Magin, R},
  journal={Communications in Nonlinear Science and Numerical Simulation},
  volume={15},
  number={4},
  pages={939--945},
  year={2010},
  publisher={Elsevier}
}

@article{lidon2017power,
  title={Power-law creep and residual stresses in a carbopol gel},
  author={Lidon, Pierre and Villa, Louis and Manneville, S{\'e}bastien},
  journal={Rheologica Acta},
  volume={56},
  number={3},
  pages={307--323},
  year={2017},
  publisher={Springer}
}

@article{friedrich1988extension,
  title={Extension of a model for crosslinking polymer at the gel point},
  author={Friedrich, CHR and Heymann, L},
  journal={Journal of Rheology},
  volume={32},
  number={3},
  pages={235--241},
  year={1988},
  publisher={SOR}
}

@article{nobile2008development,
  title={Development and rheological investigation of novel alginate/N-succinylchitosan hydrogels},
  author={Nobile, MR and Pirozzi, V and Somma, E and Gomez D'Ayala, G and Laurienzo, P},
  journal={Journal of Polymer Science Part B: Polymer Physics},
  volume={46},
  number={12},
  pages={1167--1182},
  year={2008},
  publisher={Wiley Online Library}
}

@article{blair1944study,
  title={A study of the firmness of soft materials based on Nutting's equation},
  author={Blair, GW Scott and Veinoglou, BC},
  journal={Journal of Scientific Instruments},
  volume={21},
  number={9},
  pages={149},
  year={1944},
  publisher={IOP Publishing}
}

@article{lee1998viscoelastic,
  title={Viscoelastic constitutive model for asphalt concrete under cyclic loading},
  author={Lee, Hyun-Jong and Kim, Y Richard},
  journal={Journal of engineering mechanics},
  volume={124},
  number={1},
  pages={32--40},
  year={1998},
  publisher={American Society of Civil Engineers}
}

@article{kim1995correspondence,
  title={Correspondence principle for characterization of asphalt concrete},
  author={Kim, YR and Lee, YC and Lee, HJ},
  journal={Journal of Materials in Civil Engineering},
  volume={7},
  number={1},
  pages={59--68},
  year={1995},
  publisher={American Society of Civil Engineers}
}

@article{forough2016comparing,
  title={Comparing various fitting models to construct the tensile relaxation modulus master curve of asphalt mixes},
  author={Forough, Seyed Arash and Nejad, Fereidoon Moghadas and Khodaii, Ali},
  journal={International Journal of Pavement Engineering},
  volume={17},
  number={4},
  pages={314--330},
  year={2016},
  publisher={Taylor \& Francis}
}

@article{yu2017wellbore,
  title={A wellbore creep model based on the fractional viscoelastic constitutive equation},
  author={Yu, PENG and Jinzhou, ZHAO and Yongming, LI},
  journal={Petroleum Exploration and Development},
  volume={44},
  number={6},
  pages={1038--1044},
  year={2017},
  publisher={Elsevier}
}

@article{ma2018new,
  title={A new shear rheological model for a soft interlayer with varying water content},
  author={Ma, Chong and Zhan, Hong-bin and Yao, Wen-min and Li, Hua-zhou},
  journal={Water Science and Engineering},
  volume={11},
  number={2},
  pages={131--138},
  year={2018},
  publisher={Elsevier}
}

@article{zhang2018long,
  title={A long term evaluation of circular mat foundations on clay deposits using fractional derivatives},
  author={Zhang, Cheng-Cheng and Zhu, Hong-Hu and Shi, Bin and Fatahi, Behzad},
  journal={Computers and Geotechnics},
  volume={94},
  pages={72--82},
  year={2018},
  publisher={Elsevier}
}

@article{ding2017unexpected,
  title={Unexpected viscoelastic deformation of tight sandstone: Insights and predictions from the fractional Maxwell model},
  author={Ding, Xiang and Zhang, Guangqing and Zhao, Bo and Wang, Yan},
  journal={Scientific Reports},
  volume={7},
  number={1},
  pages={11336},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{liao2017fractional,
  title={A fractional order creep constitutive model of warm frozen silt},
  author={Liao, Mengke and Lai, Yuanming and Liu, Enlong and Wan, Xusheng},
  journal={Acta Geotechnica},
  volume={12},
  number={2},
  pages={377--389},
  year={2017},
  publisher={Springer}
}

@article{lai2016investigation,
  title={Investigation progresses and applications of fractional derivative model in geotechnical engineering},
  author={Lai, Jinxing and Mao, Sheng and Qiu, Junling and Fan, Haobo and Zhang, Qian and Hu, Zhinan and Chen, Jianxun},
  journal={Mathematical Problems in Engineering},
  volume={2016},
  year={2016},
  publisher={Hindawi}
}

@article{zhang2016rheological,
  title={A rheological model to quantify strain of waxy crude oil loaded by linear increased stress},
  author={Zhang, Ze and Hou, Lei and Chen, Xuejiao and Zhou, Yayun and Liu, Mengqi and Zhou, Wenwen},
  journal={Journal of Dispersion Science and Technology},
  volume={37},
  number={3},
  pages={326--332},
  year={2016},
  publisher={Taylor \& Francis}
}

@article{hou2014new,
  title={A new approach to model strain change of gelled waxy crude oil under constant stress},
  author={Hou, Lei and Song, Changyu and Yan, Wei and Zhang, Ze},
  journal={Rheologica Acta},
  volume={53},
  number={4},
  pages={349--356},
  year={2014},
  publisher={Springer}
}

@article{wu2015improved,
  title={An improved Maxwell creep model for rock based on variable-order fractional derivatives},
  author={Wu, Fei and Liu, Jian Feng and Wang, Jun},
  journal={Environmental Earth Sciences},
  volume={73},
  number={11},
  pages={6965--6971},
  year={2015},
  publisher={Springer}
}


@article{lazaridou2007effects,
  title={Effects of hydrocolloids on dough rheology and bread quality parameters in gluten-free formulations},
  author={Lazaridou, Athina and Duta, D and Papageorgiou, Maria and Belc, N and Biliaderis, Costas G},
  journal={Journal of food Engineering},
  volume={79},
  number={3},
  pages={1033--1047},
  year={2007},
  publisher={Elsevier}
}


@article{tanner2008bread,
  title={Bread dough rheology and recoil: I. Rheology},
  author={Tanner, Roger I and Qi, Fuzhong and Dai, Shao-Cong},
  journal={Journal of Non-Newtonian Fluid Mechanics},
  volume={148},
  number={1-3},
  pages={33--40},
  year={2008},
  publisher={Elsevier}
}



@article{bonfanti2019unified,
  title={A unified rheological model for cells and cellularised materials},
  author={Bonfanti, Alessandra and Fouchard, Jonathan and Khalilgharibi, Nargess and  Charras, Guillaume and Kabla, Alexandre},
  journal={Royal Society Open Science},
  volume={7},
  pages={190920},
  year={2020},
  publisher={Royal Society}
}



@article{moresi2007characterisation,
  title={Characterisation of alginate gels using quasi-static and dynamic methods},
  author={Moresi, Mauro and Bruno, Maria},
  journal={Journal of food engineering},
  volume={82},
  number={3},
  pages={298--309},
  year={2007},
  publisher={Elsevier}
}

@article{mackay2018importance,
  title={The importance of rheological behavior in the additive manufacturing technique material extrusion},
  author={Mackay, Michael E},
  journal={Journal of Rheology},
  volume={62},
  number={6},
  pages={1549--1561},
  year={2018},
  publisher={SOR}
}

@article{corker20193d,
  title={3D printing with 2D colloids: designing rheology protocols to predict ‘printability’of soft-materials},
  author={Corker, Andrew and Ng, Henry C-H and Poole, Robert J and Garc{\'\i}a-Tu{\~n}{\'o}n, Esther},
  journal={Soft matter},
  volume={15},
  number={6},
  pages={1444--1456},
  year={2019},
  publisher={Royal Society of Chemistry}
}

@article{hata1968effect,
  title={Effect of plasticizers on the viscoelastic properties of poly (vinyl chloride)},
  author={Hata, N and Tobolsky, AV and Bondi, A},
  journal={Journal of Applied Polymer Science},
  volume={12},
  number={12},
  pages={2597--2613},
  year={1968},
  publisher={Wiley Online Library}
}

@article{van2010decoding,
  title={Decoding the viscoelastic response of polydisperse star/linear polymer blends},
  author={van Ruymbeke, Evelyne and Coppola, Salvatore and Balacca, Letizia and Righi, Sandra and Vlassopoulos, Dimitris},
  journal={Journal of Rheology},
  volume={54},
  number={3},
  pages={507--538},
  year={2010},
  publisher={SOR}
}

@article{laronda2017bioprosthetic,
  title={A bioprosthetic ovary created using 3D printed microporous scaffolds restores ovarian function in sterilized mice},
  author={Laronda, Monica M and Rutz, Alexandra L and Xiao, Shuo and Whelan, Kelly A and Duncan, Francesca E and Roth, Eric W and Woodruff, Teresa K and Shah, Ramille N},
  journal={Nature communications},
  volume={8},
  pages={15261},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{montarnal2011silica,
  title={Silica-like malleable materials from permanent organic networks},
  author={Montarnal, Damien and Capelot, Mathieu and Tournilhac, Fran{\c{c}}ois and Leibler, Ludwik},
  journal={Science},
  volume={334},
  number={6058},
  pages={965--968},
  year={2011},
  publisher={American Association for the Advancement of Science}
}

@article{wang2015temperature,
  title={Temperature dependence of creep and recovery behaviors of polymer composites filled with chemically reduced graphene oxide},
  author={Wang, Xu and Gong, Li-Xiu and Tang, Long-Cheng and Peng, Ke and Pei, Yong-Bing and Zhao, Li and Wu, Lian-Bin and Jiang, Jian-Xiong},
  journal={Composites Part A: Applied Science and Manufacturing},
  volume={69},
  pages={288--298},
  year={2015},
  publisher={Elsevier}
}

@article{liu2016preparation,
  title={Preparation, microstructure and rheological properties of asphalt sealants for bridge expansion joints},
  author={Liu, Shuang and Mo, Liantong and Wang, Kai and Xie, Yanjun and Woldekidan, MF},
  journal={Construction and Building Materials},
  volume={105},
  pages={1--13},
  year={2016},
  publisher={Elsevier}
}


@article{faber2017describing,
  title={Describing the firmness, springiness and rubberiness of food gels using fractional calculus. Part II: Measurements on semi-hard cheese},
  author={Faber, TJ and Jaishankar, A and McKinley, GH},
  journal={Food Hydrocolloids},
  volume={62},
  pages={325--339},
  year={2017},
  publisher={Elsevier}
}

@article{xu2011stress,
  title={A stress relaxation model for the viscoelastic solids based on the steady-state creep equation},
  author={Xu, Xianzhong and Hou, Jinping},
  journal={Mechanics of Time-Dependent Materials},
  volume={15},
  number={1},
  pages={29--39},
  year={2011},
  publisher={Springer}
}

@article{figueroa2012stress,
  title={Stress relaxation of wheat kernels and their relationship with milling, rheological, and breadmaking quality of wheat},
  author={Figueroa, JDC and Manuel, CI and Hern{\'a}ndez-Estrada, ZJ and Ram{\'\i}rez-Wong, B},
  journal={Cereal chemistry},
  volume={89},
  number={4},
  pages={211--216},
  year={2012},
  publisher={Wiley Online Library}
}



@article{gagnon2013undulatory,
  title={Undulatory swimming in fluids with polymer networks},
  author={Gagnon, DA and Shen, XN and Arratia, PE},
  journal={EPL (Europhysics Letters)},
  volume={104},
  number={1},
  pages={14004},
  year={2013},
  publisher={IOP Publishing}
}

@article{nicolle2010strain,
  title={A strain-hardening bi-power law for the nonlinear behaviour of biological soft tissues},
  author={Nicolle, St{\'e}phane and Vezin, Philippe and Palierne, J-F},
  journal={Journal of biomechanics},
  volume={43},
  number={5},
  pages={927--932},
  year={2010},
  publisher={Elsevier}
}

@article{trepat2004viscoelasticity,
  title={Viscoelasticity of human alveolar epithelial cells subjected to stretch},
  author={Trepat, Xavier and Grabulosa, Mireia and Puig, Ferranda and Maksym, Geoffrey N and Navajas, Daniel and Farr{\'e}, Ramon},
  journal={American Journal of Physiology-Lung Cellular and Molecular Physiology},
  volume={287},
  number={5},
  pages={L1025--L1034},
  year={2004},
  publisher={American Physiological Society}
}


@article{lefebvre2007pattern,
  title={The pattern of the linear viscoelastic behaviour of wheat flour dough as delineated from the effects of water content and high molecular weight glutenin subunits composition},
  author={Lefebvre, J and Mahmoudi, N},
  journal={Journal of cereal science},
  volume={45},
  number={1},
  pages={49--58},
  year={2007},
  publisher={Elsevier}
}

@article{brutman2014polylactide,
  title={Polylactide vitrimers},
  author={Brutman, Jacob P and Delgado, Paula A and Hillmyer, Marc A},
  journal={ACS Macro letters},
  volume={3},
  number={7},
  pages={607--610},
  year={2014},
  publisher={ACS Publications}
}

@article{coussot2009fractional,
  title={Fractional derivative models for ultrasonic characterization of polymer and breast tissue viscoelasticity},
  author={Coussot, Cecile and Kalyanam, Sureshkumar and Yapp, Rebecca and Insana, Michael F},
  journal={IEEE transactions on ultrasonics, ferroelectrics, and frequency control},
  volume={56},
  number={4},
  pages={715--726},
  year={2009},
  publisher={IEEE}
}

@article{blair1947limitations,
  title={Limitations of the Newtonian time scale in relation to non-equilibrium rheological states and a theory of quasi-properties},
  author={Blair, GW Scott and Veinoglou, BC and Caffyn, JE},
  journal={Proceedings of the Royal Society of London. Series A. Mathematical and Physical Sciences},
  volume={189},
  number={1016},
  pages={69--87},
  year={1947},
  publisher={The Royal Society London}
}

@book{lakes2009viscoelastic,
  title={Viscoelastic materials},
  author={Lakes, Roderic and Lakes, Roderic S},
  year={2009},
  publisher={Cambridge University Press}
}

@article{wu2018comparison,
  title={A comparison of methods to assess cell mechanical properties},
  author={Wu, Pei-Hsun and Aroush, Dikla Raz-Ben and Asnacios, Atef and Chen, Wei-Chiang and Dokukin, Maxim E and Doss, Bryant L and Durand-Smet, Pauline and Ekpenyong, Andrew and Guck, Jochen and Guz, Nataliia V and others},
  journal={Nature methods},
  volume={15},
  pages={491--498},
  year={2018},
  publisher={Springer}
}

@book{rudolf2000applications,
  title={Applications of fractional calculus in physics},
  author={Rudolf, Hilfer},
  year={2000},
  publisher={World Scientific}
}

@book{magin2006fractional,
  title={Fractional calculus in bioengineering},
  author={Magin, Richard L},
  year={2006},
  publisher={Begell House Redding}
}

@incollection{gutierrez2014constitutive,
  title={Constitutive equations in hereditary integral form},
  author={Gutierrez-Lemini, Danton},
  booktitle={Engineering Viscoelasticity},
  pages={23--52},
  year={2014},
  publisher={Springer}
}

@book{christensen2012theory,
  title={Theory of viscoelasticity: an introduction},
  author={Christensen, Richard},
  year={2012},
  publisher={Elsevier}
}

@article{ekpenyong2012viscoelastic,
  title={Viscoelastic properties of differentiating blood cells are fate-and function-dependent},
  author={Ekpenyong, Andrew E and Whyte, Graeme and Chalut, Kevin and Pagliara, Stefano and Lautenschl{\"a}ger, Franziska and Fiddler, Christine and Paschke, Stephan and Keyser, Ulrich F and Chilvers, Edwin R and Guck, Jochen},
  journal={PloS one},
  volume={7},
  number={9},
  pages={e45237},
  year={2012},
  publisher={Public Library of Science}
}

@book{podlubny1998fractional,
  title={Fractional differential equations: an introduction to fractional derivatives, fractional differential equations, to methods of their solution and some of their applications},
  author={Podlubny, Igor},
  volume={198},
  year={1998},
  publisher={Elsevier}
}

@article{surguladze2002certain,
  title={On certain applications of fractional calculus to viscoelasticity},
  author={Surguladze, TA},
  journal={Journal of Mathematical sciences},
  volume={112},
  number={5},
  pages={4517--4557},
  year={2002},
  publisher={Springer}
}


@incollection{winter1997rheology,
  title={Rheology of polymers near liquid-solid transitions},
  author={Winter, Horst Henning and Mours, Marian},
  booktitle={Neutron spin echo spectroscopy viscoelasticity rheology},
  pages={165--234},
  year={1997},
  publisher={Springer}
}


@article{beylkin2005approximation,
  title={On approximation of functions by exponential sums},
  author={Beylkin, Gregory and Monz{\'o}n, Lucas},
  journal={Applied and Computational Harmonic Analysis},
  volume={19},
  number={1},
  pages={17--48},
  year={2005},
  publisher={Elsevier}
}

@article{svensson1973approximation,
  title={An approximation method for time domain synthesis of linear networks},
  author={Svensson, Tommy},
  journal={IEEE Transactions on Circuit Theory},
  volume={20},
  number={2},
  pages={142--144},
  year={1973},
  publisher={IEEE}
}


@book{odian2004principles,
  title={Principles of polymerization},
  author={Odian, George and others},
  year={2004},
  publisher={John Wiley \& Sons}
}


@article{friedrich1991relaxation,
  title={Relaxation and retardation functions of the Maxwell model with fractional derivatives},
  author={Friedrich, CHR},
  journal={Rheologica Acta},
  volume={30},
  number={2},
  pages={151--158},
  year={1991},
  publisher={Springer}
}

@book{kailath1980linear,
  title={Linear systems},
  author={Kailath, Thomas},
  volume={156},
  year={1980},
  publisher={Prentice-Hall Englewood Cliffs, NJ}
}

@inproceedings{gorenflo2002computation,
  title={Computation of the Mittag-Leffler function E$\alpha$, $\beta$ (z) and its derivative},
  author={Gorenflo, Rudolf and Loutchko, Joulia and Luchko, Yuri},
  booktitle={Fract. Calc. Appl. Anal},
  year={2002},
  organization={Citeseer}
}

@article{haubold2011mittag,
  title={Mittag-Leffler functions and their applications},
  author={Haubold, Hans J and Mathai, Arak M and Saxena, Ram K},
  journal={Journal of Applied Mathematics},
  volume={2011},
  year={2011},
  publisher={Hindawi}
}

@article{park2010measurement,
  title={Measurement of red blood cell mechanics during morphological changes},
  author={Park, YongKeun and Best, Catherine A and Badizadegan, Kamran and Dasari, Ramachandra R and Feld, Michael S and Kuriabova, Tatiana and Henle, Mark L and Levine, Alex J and Popescu, Gabriel},
  journal={Proceedings of the National Academy of Sciences},
  volume={107},
  number={15},
  pages={6731--6736},
  year={2010},
  publisher={National Acad Sciences}
}

@article{sun2012mechanics,
  title={Mechanics regulates fate decisions of human embryonic stem cells},
  author={Sun, Yubing and Villa-Diaz, Luis G and Lam, Raymond HW and Chen, Weiqiang and Krebsbach, Paul H and Fu, Jianping},
  journal={PloS one},
  volume={7},
  number={5},
  pages={e37178},
  year={2012},
  publisher={Public Library of Science}
}

@article{messal2019tissue,
  title={Tissue curvature and apicobasal mechanical tension imbalance instruct cancer morphogenesis},
  author={Messal, Hendrik A and Alt, Silvanus and Ferreira, Rute MM and Gribben, Christopher and Wang, Victoria Min-Yi and Cotoi, Corina G and Salbreux, Guillaume and Behrens, Axel},
  journal={Nature},
  volume={566},
  number={7742},
  pages={126},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{tripathi2010peristaltic,
  title={Peristaltic flow of viscoelastic fluid with fractional Maxwell model through a channel},
  author={Tripathi, D and Pandey, SK and Das, S},
  journal={Applied Mathematics and Computation},
  volume={215},
  number={10},
  pages={3645--3654},
  year={2010},
  publisher={Elsevier}
}

@article{celauro2012experimental,
  title={Experimental validation of a fractional model for creep/recovery testing of asphalt mixtures},
  author={Celauro, C and Fecarotti, C and Pirrotta, A and Collop, AC},
  journal={Construction and Building Materials},
  volume={36},
  pages={458--466},
  year={2012},
  publisher={Elsevier}
}


@article{kaplan2019pectin,
  title={On Pectin Methyl-esterification: Implications for In vitro and In vivo Viscoelasticity},
  author={Kaplan, J Louis and Torode, Thomas A and Daher, Firas Bou and Braybrook, Siobhan A},
  journal={bioRxiv},
  pages={565614},
  year={2019},
  publisher={Cold Spring Harbor Laboratory}
}


@article{kaplanrheos,
	title = {{RHEOS}.jl -- {A} {Julia} {Package} for {Rheology} {Data} {Analysis}},
	journal = {Journal of Open Source Software},
	author = {Kaplan, J Louis and Bonfanti, Alessandra and Kabla, Alexandre},
	year = {2019},
}

@book{oldham1974fractional,
  title={The fractional calculus theory and applications of differentiation and integration to arbitrary order},
  author={Oldham, Keith and Spanier, Jerome},
  volume={111},
  year={1974},
  publisher={Elsevier}
}


@article{pritchard2017oscillations,
  title={Oscillations and damping in the fractional Maxwell materials},
  author={Pritchard, Robyn H and Terentjev, Eugene M},
  journal={Journal of Rheology},
  volume={61},
  number={2},
  pages={187--203},
  year={2017},
  publisher={SOR}
}

@article{mainardi2011creep,
  title={Creep, relaxation and viscosity properties for basic fractional models in rheology},
  author={Mainardi, Francesco and Spada, Giorgio},
  journal={The European Physical Journal Special Topics},
  volume={193},
  number={1},
  pages={133--160},
  year={2011},
  publisher={Springer}
}

@article{shen2013fractional,
  title={Fractional order viscoelasticity in characterization for atrial tissue},
  author={Shen, Jing Jin and Li, Cheng Gang and Wu, Hong Tao and Kalantari, Masoud},
  journal={Korea-Australia Rheology Journal},
  volume={25},
  number={2},
  pages={87--93},
  year={2013},
  publisher={Springer}
}

@article{holder2018control,
  title={Control of collagen gel mechanical properties through manipulation of gelation conditions near the sol--gel transition},
  author={Holder, AJ and Badiei, N and Hawkins, K and Wright, C and Williams, PR and Curtis, DJ},
  journal={Soft matter},
  volume={14},
  number={4},
  pages={574--580},
  year={2018},
  publisher={Royal Society of Chemistry}
}

@article{keshavarz2017nonlinear,
  title={Nonlinear viscoelasticity and generalized failure criterion for polymer gels},
  author={Keshavarz, Bavand and Divoux, Thibaut and Manneville, S{\'e}bastien and McKinley, Gareth H},
  journal={ACS Macro Letters},
  volume={6},
  number={7},
  pages={663--667},
  year={2017},
  publisher={ACS Publications}
}


@article{muller2011nonlinear,
  title={A nonlinear fractional viscoelastic material model for polymers},
  author={M{\"u}ller, Sebastian and K{\"a}stner, Markus and Brummund, J{\"o}rg and Ulbricht, Volker},
  journal={Computational Materials Science},
  volume={50},
  number={10},
  pages={2938--2949},
  year={2011},
  publisher={Elsevier}
}

@article{bharadwaj2017strain,
  title={A strain stiffening theory for transient polymer networks under asymptotically nonlinear oscillatory shear},
  author={Bharadwaj, N Ashwin and Schweizer, Kenneth S and Ewoldt, Randy H},
  journal={Journal of Rheology},
  volume={61},
  number={4},
  pages={643--665},
  year={2017},
  publisher={Society of Rheology}
}

